Convergence Rates for Empirical Estimation of Binary Classification Bounds

Bounding the best achievable error probability for binary classification problems is relevant to many applications including machine learning, signal processing, and information theory. Many bounds on the Bayes binary classification error rate depend on information divergences between the pair of class distributions. Recently, the Henze-Penrose (HP) divergence has been proposed for bounding classification error probability. We consider the problem of empirically estimating the HP-divergence from random samples. We derive a bound on the convergence rate for the Friedman-Rafsky (FR) estimator of the HP-divergence, which is related to a multivariate runs statistic for testing between two distributions. The FR estimator is derived from a multicolored Euclidean minimal spanning tree (MST) that spans the merged samples. We obtain a concentration inequality for the Friedman-Rafsky estimator of the Henze-Penrose divergence. We validate our results experimentally and illustrate their application to real datasets.

==> Ref.tex <==
%\begin{thebibliography}{9}

\bibitem{AS}
\textsc{Ali, S. and Silvey, S.D.} (1996). A general class of coefficients of divergence of one distribution from another. \textit{J. Royal Statist. Soc. Ser. B (Methodology.)} 131--142. 

%\bibitem{AID}
%\textsc{Avi-Itzhak, H. and Diep, T.} (1996). Arbitrarily tight upper and lower bounds on the Bayesian probability of error. {\it IEEE Trans. Pattern Anal. Mach. Intell.} Vol. \textbf{18}, no. \textbf{1} 89--91. 

\bibitem{ADS}
\textsc{Avis, D., Davis, B. and Steele, J.M.} (1988). Probabilistic analysis of a greedy heuristic for Euclidean matching. {\it Probability in the Engineering and Information Sciences} \textbf{2} 143--156. 


\bibitem{BLJN}
\textsc{Banks, D., Lavine, M. and Newton, H.J.} (1992). The minimal spanning tree for nonparametric regression and structure discovery. in {\it computing Science and Statistics. Proceedings of the 24th Symposium on the Interface}, H. Joseph Newton, Ed., 370--374.

\bibitem{Ba}
\textsc{Basseville, M.} (2013) Divergence measures for statistical data processing--An annotated bibliography. {\it Signal Processing}. Vol. \textbf{93}, no. \textbf{4} 621--633. 

\bibitem{Bha}
\textsc{Battacharyya, A.} (1946). On a measure of divergence between two multinomial populations. \textit{Sankhy \={a}: The Indian Journal of Statistics}. 401--406.

\bibitem{BH}
\textsc{Berisha V. and Hero, A.O.} (2015). Empirical non-parametric estimation of the Fisher information. \textit{IEEE Signal Process. Lett.} Vol. \textbf{22}, no. \textbf{7} 988--992.


\bibitem{BWHS}
\textsc{Berisha, V., Wisler, A., Hero, A.O. and Spanias, A.}. (2016). Empirically estimable classification bounds based on a nonparametric divergence measure. {\it IEEE Trans. on Signal Process.} Vol. \textbf{64}, no. \textbf{3} 580--591.


\bibitem{Cha}
\textsc{Cha, S.H.} (2007). Comprehensive survey on distance/similarity measures between probability density functions. {\it Int. J. Math. Models Methods Appl. Sci.} Vol. \textbf{1}, no. \textbf{4} 300--307. 


%\bibitem{Che}
%\textsc{Chernoff, H.} (1952). A measure of asymptotic efficiency for tests of a hypothesis based on the sum of observations. {\it The Annals of Mathematical Statistics} 493--507.


%\bibitem{Cs}
%\textsc{Csiszar, I.} (1967). Infomration-type measures of difference of probability distributions and indirect observations. {\it Studia Sci. Math. Hungar.} Vol. \textbf{2} 299--318. 


\bibitem{ES}
\textsc{Efron, B. and stein, C.} (1981). The jackknife estimate of variance. {\it Annals of Statistics} \textbf{9} 586--596. 


\bibitem{FR}
\textsc{Friedman, J.H. and Rafsky, L.C.} (1979). Multivariate generalizations of the Wald-Wolfowitz and Smirnov two-sample tests, {\it Ann. Statist.} 697--717. 



\bibitem{Gi}
\textsc{Gibbons, J.D.} (1971). \textit{Nonparametric Statistical Inference}, McGraw-Hill.  

\bibitem{ref6}
\textsc{Guorong, X., Peiqi,C. and Minhui, W.} (1996). \textit{Bhattacharyya distance feature
selection.} In Pattern Recognition, Proceedings of the 13th International Conference on IEEE, vol. \textbf{2} 195--199.


\bibitem{ref7}
\textsc{Hamza, A.B. and Krim, H.} (2003). Image registration and segmentation
by maximizing the Jensen-Renyi divergence. {\it  Energy Minimization
Methods in Computer Vision and Pattern Recognition}. Springer 147--163.


%\bibitem{HVS}
%\textsc{Hashlamoun, W.A., Varshney, P.K. and Samarasooriya, V.} (1994). A tight upper bound on the Bayesian probability of error. {\it IEEE Trans. Pattern Anal. Mach. Intell.} Vol. \textbf{16}, no. \textbf{2} 220--224. 


\bibitem{HHC}
\textsc{Heemuchwala, H., Hero, A.O. and Carson, P.} (2003). Image registration using entropy measures and entropic graphs. {\it European Journal of Signal Processing, Special Issue on Content-based Visual Information Retrieval}.



%\bibitem{He}
%\textsc{Hellinger, E.} (1909). Neue Begr\''{u}ndung der theorie quadratischer formen von unendlichvielen ver\"{a}nderlichen. {\it Journal f\"{u}r die reine und angewandte Mathematik}. Vol. \textbf{136} 210--271.



%\bibitem{HR}
%\textsc{Hellman, M.E. and Raviv, J.} (1970). Probability of error, equivocation, and the Chernoff bound. {\it IEEE Trans. on Infom. Theory}. Vol. \textbf{IT-16}, no. \textbf{4} 368--372. 



\bibitem{HP}
\textsc{Henze, N. and Penrose, M.D.} (1999). On the multivarite runs test. {\it Ann. Statist.} Vol. \textbf{27}, no. \textbf{1} 290--298. 


\bibitem{HCM}
\textsc{Hero, A.O., Costa, J.A. and Ma, B.} (2003). Convergence rates of minimal graphs with random vertices. {\it http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.8.4480 rep=rep1 type=pdf}.


\bibitem{HCB}
\textsc{Hero, A.O., Costa, J.A. and Ma, B.} (2003). Asymptotic relations between minimal graphs and alpha-entropy. {\it Comm. and Sig. Proc. Lab.(CSPL), Dept. EECS, University of Michigan, Ann Arbor, Tech. Rep.}



%\bibitem{HMMG}
%\textsc{Hero, A.O., Ma, B., Michel, O. and Gorman, J.} (2001). {\it Alpha-divergence for classification, indexing and retrieval}. Communication and Signal  Processing Laboratory, Technical Report CSPL-328, U. Mich. 


\bibitem{HMMG}
\textsc{Hero, A.O., Ma, B., Michel, O. and Gorman, J.} (2002). Applications of entropic spanning graphs. {\it IEEE Signal Processing Magazine}. Vol. \textbf{19}, no. \textbf{5} 85--95. 



\bibitem{HM}
\textsc{Hero, A.O. and Michel, O.} (1999). Estimation of R\'{e}nyi information divergence via pruned minimal spanning trees. in {\it IEEE Workshop on Higher Order Statistics}, Carsaria, Isreal.


\bibitem{ref8}
\textsc{Hild, K. E., Erdogmus, D. and Principe, J. C.}(2001). Blind source separation using Renyi's mutual information. {\it  Signal Processing Letters, IEEE},
vol. \textbf{8}, no. \textbf{6} 174--176.


\bibitem{HJ}
\textsc{Hoffman, R. and Jain, A.K.} (1983). A test of randomness based on the minimal spanning tree. {\it Pattern Recognition Letters}. Vol. \textbf{1} 175--180.


%\bibitem{Ka}
%\textsc{Kailath, T.} (1967). The divergence and Battacharyya distance measure in signal selection. {\it IEEE Trans. Commun, Technol.}, Vol. \textbf{15}, no. \textbf{1} 52--60. 


\bibitem{KKPWR}
\textsc{Kandasamy, K., Krishnamurthy, A., P\'{o}czos, B., Wasserman, L. and Robins, J.} (2015). Nonparametric von mises estimators for entropies, divergence and mutual informations, in {\it Advances in Neural Information Processing Systems} 397--405. 


%\bibitem{KFG}
%\textsc{Khosravifard,M., Fooladivanda, D. and Gulliver, T.A.} (2007). Conáiction of the convexity and metric properties in $f$-divergences. {\it IEICE-Tran. Fund. Elec. Comm. Comp. Sci.} E90-A. 1848--1853.

\bibitem{Ki}
\textsc{Kingman, J.F.C.} (1993). {\it Poisson Processes}. Oxford Univ. Press. 


%\bibitem{KKPW}
%\textsc{Krishnamurthy, A., Kandasamy, K., P\'{o}czos, B. and Wasserman, L.} (2014). Nonparametric estimation of Renyi divergence and friends, in {\it Proceedings of the 31st International Conference on Machine Learning} 919--927. 


\bibitem{KL}
\textsc{Kullback, S. and Leibler, R.A.} (1951). On information and sufficiency. {\it The annals of Mathematical Statistics}. Vol. \textbf{22}, no. \textbf{1} 79--86. 

\bibitem{Lo}
\textsc{ Lorentz, G.G.} (1966). {\it Approximation of functions}. Holt, Rinehart and Winston, New York/Chicago/Toronto. 


\bibitem{MHGM}
\textsc{Ma, B., Hero, A.O., Gorman, J. and Michel, O.} (2000). Image registration with minimal spanning tree algorithm. {\it IEEE Int. Conf. on Image Processing}, Vancouver, BC.  

%\bibitem{MMR}
%\textsc{Mansour, Y., Mohri, M. and Rostamizadeh, A.} (2009).  {\it Proc. Domain Adaptation: Learning Bounds and Algorithms}. Available: arXiv preprint arXive:0902.3430. 


\bibitem{MH}
\textsc{Moon, K.R. and Hero, A.O.} (2014). Multivariate $f$-divergence estimation with confidence. in {\it Proc. Adv. Neural Inf. Process. Syst.} 2420--2428.


\bibitem{Moon2014ISIT}
\textsc{Moon, K.R. and Hero, A.O} (2014). Ensemble estimation of multivariate f-divergence. {\it IEEE International Symposium on Information Theory (ISIT)} 356--360. 


\bibitem{Moon2016ISIT}
\textsc{Moon, K.R, Sricharan, K., Greenewald, K. and Hero, A.O.} (2016). Improving convergence of divergence functional ensemble estimators. {\it IEEE International Symposium on Information Theory (ISIT)} 1133--1137.


\bibitem{MSGH}
\textsc{Moon, K.R, Sricharan, K., Greenewald, K. and Hero, A.O.} (2016). Nonparametric ensemble estimation of distributional functionals. {\it arXiv preprint arXiv: 1601.06884v2}. 


\bibitem{NMYH}
\textsc{Noshad, M., Moon, K.R., Yasaei Sekeh, S. and Hero, A.O.} (2017). Direct Estimation of Information Divergence Using Nearest Neighbor Ratios. {\it IEEE International Symposium on Information Theory (ISIT)}. 


\bibitem{YOH}
\textsc{Yasaei Sekeh, S., Oselio, B. and Hero, A.O.} (2018). A Dimension-Independent discriminant between distributions. in {\it proc. IEEE Int. Conf. on Image Processing (ICASSP).}


\bibitem{PPS}
\textsc{P\'{a}l, D., P\'{o}czos, B. and Szapesv\'{a}ri, C.} (2010). Estimation of Renyi entropy and mutual information based on generalized nearest-neighbor graphs. {\it NIPS 23}.  


%\bibitem{RP}
%\textsc{Ramaswamy, S.I. and Patki, R.} (2015). Distributed Minimum Spanning Trees
% . {\it Available in https://stanford.edu/rezab/classes/cme323/S15/projects/distributed minimum spanning trees report.pdf}.  
 

\bibitem{RY}
\textsc{Redmond, C. and Yukich, J.E.} (1994). Limit theorems and rates of convergence for Euclidean functionals. {\it Ann. Applied Probab.} Vol. \textbf{4}, no. \textbf{4} 1057--1073. 


\bibitem{RY1}
\textsc{Redmond, C. and Yukich, J.E.} (1996). Asymptotics for Euclidean functionals with power weighted edges. {\it Stochastic Processes and their Applications}. Vol. \textbf{6} 289--304.



\bibitem{R}
\textsc{R\'{e}nyi, A.} (1961). On measures of entropy and information. in {\it Fourth Berkeley Sympos. on Mathematical Stat. and Prob.} 547--561. 



\bibitem{Rh1993b}
\textsc{Rhee, W.} (1993b). A matching problem and subadditive Euclidean funetionals. {\it Ann. Appl. Prob.,} \textbf{3} 794--801. 

\bibitem{ZHR}
\textsc{Zhang, Y., Hero, A.O. and Rogers, W.L.} (1994). Simultaneous Confidence Intervals for Image Reconstruction Problems. in {\it Proceedings of the IEEE International Conference on  Acoustics, Speech, and Signal Processing (ICASSP-94)}. 


\bibitem{Ru}
\textsc{Rukhin, A.} (1994). Optimal estimator for the mixture parameter by the method of moments and information affinity. in {\it Proc. Trans. 12th Prague Conf. Inf. Theory} 214--219. 




\bibitem{SP}
\textsc{Singh, S. and P\'{o}czos, B.} (2014). Generalized exponential concentration inequality for Renyi divergence estimation, in {\it Proceedings of the 31st International Conference on Machine Learning (ICML-14)} 333--341. 


\bibitem{SP2}
\textsc{Singh, S. and P\'{o}czos, B.} (2014). Exponential concentration of a density functional estimator. in {\it Advances in Neural Information Processing Systems} 3032--3040.


\bibitem{Sm}
\textsc{Smirnov, N.V.} (1939). On the estimation of the discrepancy between empirical curves of distribution for two independent samples. {\it Bull. Moscow Univ.} \textbf{2} 3--6. 



%\bibitem{SWH}
%\textsc{Sricharan, K., Wei, D. and Hero, A.O.} (2013). Ensemble estimation for multivariate entropy estimation. {\it IEEE Trans. on Inform. Theo.} Vol. \textbf{59}, no. \textbf{7} 4374--4388.


\bibitem{St1997}
\textsc{Steele, J.M.} (1997). Probability Theory and Combinatorial Optimization. Vol. \textbf{69} of {\it CBMF-NSF regional conference in applied mathematics}, Society for Industrial and Applied Mathematics (SIAM). 



\bibitem{Steele1986}
\textsc{Steele, J.M.} (1986). An Efron-Stein inequality for nonsymmetric statistics. {\it Annals of Statistics} \textbf{14} 753--758. 


\bibitem{St1988}
\textsc{Steele, J.M.} (1998). Growth rates of Euclidean minimal spanning trees with power weighted edges. {\it Ann. Prob.,} \textbf{16} 1767--1787. 


\bibitem{SSE}
\textsc{Steele, J.M., Shepp, L.A. and Eddy, W.F.} (1987). On the number of leaves of a euclidean minimal spanning tree. {\it J. Appl. Prob.} \textbf{24} 809--826. 



\bibitem{Ta}
\textsc{Talagrand, M.} (1995). Concentration of measure and isoperimetric inequalities in product spaces. {\it Publications Math\'{e}matiques de i'I. H. E. S.} \textbf{81} 73--205. 


\bibitem{To}
\textsc{Toussaint, G.T.} (1980). The relative neighborhood graph of a finite planar set. {\it Pattern Recognition}. Vol. \textbf{12} 261--268. 


\bibitem{Yu}
\textsc{Yukich, J.E.} (1998).  {\it Probability theory of classical Euclidean optimization}, vol. 1675 of Lecture Notes in Mathematics, Springer-Verlag, Berlin.



\bibitem{WW0}
\textsc{Wald, A. and Wolfowitz, J.} (1940). On a test whether two samples are from the same population. {\it Ann. Math. Statist.} \textbf{11} 147--162. 



%\bibitem{WKV0}
%\textsc{Wang, Q., Kulkarni, S.R. and Verd\'{u}, S.} (2005). Divergence Estimation of Continuous Distributions. {\it IEEE Transactions on Information Theory}. Vol. \textbf{51}, no. \textbf{9} 3064--3074. 



%\bibitem{WKV}
%\textsc{Wang, Q., Kulkarni, S.R. and Verd\'{u}, S.} (2009). Divergence estimation for multidimensional densities via k-nearest-neighbor distances. {\it IEEE Trans. Information Theory}. Vol. \textbf{55}, no. \textbf{5} 2392--2405. 


\bibitem{WW}
\textsc{Whittaker, E.T. and Watson, G.N.} (1996). {\it A Course in Modern Analysis (4th ed.)}, New York: Cambridge University Press.  


\bibitem{WBWRS}
\textsc{Wisler, A., Berisha, V., Wei, D., Ramamurthy, K. and Spanias, A.} (2016). Empirically-estimable multi-class classification bounds. {\it IEEE International Conference on Acoustics, Speech and Signal Processing}. 



\bibitem{Za}
\textsc{Zahn, C.T.} (1971). Graph-theoretical methods for detecting and describing Gestalt clusters. {\it IEEE Trans. on Computers}. Vol. \textbf{C-20} 68--86. 

\bibitem{UCI}
M. Lichman, “UCI machine learning repository,” 2013.

\bibitem{SKIN}
 Rajen B. Bhatt, Gaurav Sharma, Abhinav Dhall, Santanu Chaudhury. Efficient skin region segmentation using low complexity fuzzy decision tree model, {\it IEEE-INDICON} 2009, Dec 16-18, Ahmedabad, India, 1--4.

%-----------------------------------------------------------





%\bibitem{KKT}
%D. Karger, P. Klein and R. Tarjan, A randomized linear-time algorithm to find minimum spanning trees, {\it Journal of the Association for Computing Machinery}, vol 42, No 2, pp. 321-328, 1995. 

%\bibitem{Pri}
%R. C. Prim, {\it Shortest connection networks And some generalizations}, Bell System Technical Journal, 36 (6), pp. 1389-1401, 1957. 

%\bibitem{MRG}
%W. March, P. Ram and A G. Gary, Fast Euclidean minimum spanning tree: algorithm, analysis and applications, {\it Proceeding KDD '10 Proceedings of the 16th ACM SIGKDD international conference on Knowledge discovery and data mining}, pp. 603-612, 2010. 

%\bibitem{Tsai}
%Y. Tsai, A randomized algorithm to find minimum spanning tree, {\it Technical Report}, Dec 5, 2013. 
%--------------------------------------------








%\end{thebibliography}

